Synchronization of Multiple Videos

Synchronizing videos captured simultaneously from multiple cameras in the same scene is often easy and typically requires only simple time shifts. However, synchronizing videos from different scenes or, more recently, generative AI videos, poses a far more complex challenge due to diverse subjects, backgrounds, and nonlinear temporal misalignment. We propose Temporal Prototype Learning (TPL), a prototype-based framework that constructs a shared, compact 1D representation from high-dimensional embeddings extracted by any of various pretrained models. TPL robustly aligns videos by learning a unified prototype sequence that anchors key action phases, thereby avoiding exhaustive pairwise matching. Our experiments show that TPL improves synchronization accuracy, efficiency, and robustness across diverse datasets, including fine-grained frame retrieval and phase classification tasks. Importantly, TPL is the first approach to mitigate synchronization issues in multiple generative AI videos depicting the same action. Our code and a new multiple video synchronization dataset are available at https://bgu-cs-vil.github.io/TPL/

==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}




\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{green}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  



\newcommand{\FREIFELD}[1]{\textbf{\MAGENTA{[FREIFELD says: #1]}}}
% Make your own

\newcommand{\TBD}{\RED{[TBD]}}
\newcommand{\TODO}[1]{\RED{[TODO: #1]}}




% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}

\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbbm{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


==> supmat/fig_joint_alignment.tex <==

\begin{figure}[h]

%\def\figwidth{0.98\textwidth}
  \centering
  \begin{subfigure}{0.49\textwidth}
  % [left, down, right, up]
    \includegraphics[trim = 5mm 0mm 5mm 12mm, clip, width=\textwidth]{../figures/baseball_swing_before.pdf}
    \caption{\emph{Baseball swing} 1-D Latent representation}
  \end{subfigure}
  %\hfill
  \begin{subfigure}{0.49\textwidth}
    \includegraphics[trim = 5mm 0mm 5mm 12mm, clip, width=\textwidth]{../figures/baseball_swing_after.pdf}
    \caption{After alignment}
  \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
  % [left, down, right, up]
    \includegraphics[trim = 5mm 0mm 5mm 12mm, clip, width=\textwidth]{../figures/golf_swing_before.pdf}
    \caption{\emph{golf swing} 1-D Latent representation}
  \end{subfigure}
  %\hfill
  \begin{subfigure}{0.49\textwidth}
    \includegraphics[trim = 5mm 0mm 5mm 12mm, clip, width=\textwidth]{../figures/golf_swing_after.pdf}
    \caption{After alignment}
  \end{subfigure}


\caption{Joint alignment of the one-dimensional representation for 20 randomly sampled videos of the \emph{Baseball swing} (top) and \emph{golf swing} (bottom) action colored by the phase labels, before (left) and after alignment (right). }\label{fig:JA:1}

\end{figure}

\newpage

==> tables/tab_penn_action.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{0em}
\centering
\caption{List of all key events in the Penn Action Datasets~\cite{zhang:ICCV:2013:penn}, which was densely annotate by~\cite{Debidatta:CVPR:2019:TCCL}. The Pouring dataset~\cite{Sermanet:ICRA:2018:pouring} appears last. Each action has a \textit{Start} event and \textit{End} event in addition to the key events.}
\footnotesize{
    \begin{tabular}{l|c|p{5.3cm}|c| c}
        \textbf{Action} & \textbf{\#phases} & \textbf{List of Key Events} & \textbf{Train set} & \textbf{Val set} \\
        \midrule
        \midrule
        Baseball Pitch & 4 & Knee fully up, Arm fully stretched out, Ball release & 103 & 63\\
        Baseball Swing & 3 & Bat swung back fully, Bat hits ball & 113 & 57\\
        Bench-press & 2 & Bar fully down & 69 & 71\\
        Bowling & 3 & Ball swung fully back, Ball release & 134 & 85\\
        Clean and jerk & 6 & Bar at hip, Fully squatting, Standing, Begin Thrusting, Beginning Balance & 40 & 42\\
        Golf swing & 3 & Stick swung fully back, Stick hits ball & 87 & 77 \\
        Jumping jacks & 4 & Hands at shoulder (going up), Hands above head, Hands at shoulders (going down) & 56 & 56\\
        Pullups & 2 & Chin above bar & 98 & 101\\
        Pushups & 2 & Head at floor & 102 & 105\\
        Situps & 2 & Abs fully crunched & 50 & 50\\
        Squats & 4 & Hips at knees (going down), Hips at floor, Hips at knee (going up) &  114 & 116\\
        Tennis forehand & 3 & Racket swung fully back, Racket touches ball & 79 & 74\\
        Tennis serve & 4 & Ball released from hand, Racket swung fully back, Ball touches racket &  115 & 69\\
        \midrule
        Pouring & 5 & Hand touches bottle, Liquid starts exiting, Pouring complete, Bottle back on table & 70 & 14\\
        \bottomrule
 
    \end{tabular}
\label{tab:penn}
}
\vspace{-1em}
\end{table}

==> tables/tab_tcc_net.tex <==
\begin{table}[h]
\centering
\footnotesize{
\caption{Architecture of the embedding network used for the initial embedding, $\phi(\cdot)$.}

\begin{tabular}{c|c|c}
\hline
Operations                  & Output Size              & Parameters\\
\hline
\hline
Temporal Stacking      & $k'\times$14$\times$14$\times$$c$        & Stack $k'$ context frames \\ 
3D Convolutions &  $k'\times$14$\times$14$\times$512 & [3$\times$3$\times$3$, $512] $\times$ 2\\
Spatio-temporal Pooling & 512 & Global 3D Max-pooling \\
Fully-connected layers & 512& [512] $\times$ 2\\
Linear projection      & 128                        & 128                                                                                    \\ \hline
\end{tabular}
\label{tab:tcc:net}
}
\end{table}
